Unpaired Optical Coherence Tomography Angiography Image Super-Resolution via Frequency-Aware Inverse-Consistency GAN

For optical coherence tomography angiography (OCTA) images, a limited scanning rate leads to a trade-off between field-of-view (FOV) and imaging resolution. Although larger FOV images may reveal more parafoveal vascular lesions, their application is greatly hampered due to lower resolution. To increase the resolution, previous works only achieved satisfactory performance by using paired data for training, but real-world applications are limited by the challenge of collecting large-scale paired images. Thus, an unpaired approach is highly demanded. Generative Adversarial Network (GAN) has been commonly used in the unpaired setting, but it may struggle to accurately preserve fine-grained capillary details, which are critical biomarkers for OCTA. In this paper, our approach aspires to preserve these details by leveraging the frequency information, which represents details as high-frequencies ($\textbf{hf}$) and coarse-grained backgrounds as low-frequencies ($\textbf{lf}$). In general, we propose a GAN-based unpaired super-resolution method for OCTA images and exceptionally emphasize $\textbf{hf}$ fine capillaries through a dual-path generator. To facilitate a precise spectrum of the reconstructed image, we also propose a frequency-aware adversarial loss for the discriminator and introduce a frequency-aware focal consistency loss for end-to-end optimization. Experiments show that our method outperforms other state-of-the-art unpaired methods both quantitatively and visually.

==> paper/6_prev_conclusion.tex <==
\section{Conclusion}
This paper presented a novel approach, Frequency-aware Unpaired Super-Resolution for OCTA images (FUSR), for enhancing the resolution using the unpaired setting. We proposed a GAN-based framework to mimic restoration and degradation mappings, optimized end-to-end through consistency loss. Given the importance of fine-grained capillaries in microvasculature as biomarkers for OCTA, we employed frequency decomposition to emphasize $hf$ by separating and fusing frequency components. We also introduced an \textbf{FAL} for the discriminators to better preserve the capillary structure, and an \textbf{FFCL} to preserve the spectrum consistency. We conducted experiments and analytical studies to validate the effectiveness of the method and to show the superior performance. To the best of our knowledge, as an extension of our previous work~\cite{zhang2022frequency}, our studies were the first to leverage frequency analysis and to utilize GAN in unpaired OCTA super-resolution. It addressed challenges associated with large-scale data collection and complex data preparation required in conventional supervised super-resolution methods in the perspective of frequency-domain analysis.




